Pseudo-keypoint RKHS Learning for Self-supervised 6DoF Pose Estimation

We address the simulation-to-real domain gap in six degree-of-freedom pose estimation (6DoF PE), and propose a novel self-supervised keypoint voting-based 6DoF PE framework, effectively narrowing this gap using a learnable kernel in RKHS. We formulate this domain gap as a distance in high-dimensional feature space, distinct from previous iterative matching methods. We propose an adapter network, which is pre-trained on purely synthetic data with synthetic ground truth poses, and which evolves the network parameters from this source synthetic domain to the target real domain. Importantly, the real data training only uses pseudo-poses estimated by pseudo-keypoints, and thereby requires no real ground truth data annotations. Our proposed method is called RKHSPose, and achieves state-of-the-art performance among self-supervised methods on three commonly used 6DoF PE datasets including LINEMOD (+4.2%), Occlusion LINEMOD (+2%), and YCB-Video (+3%). It also compares favorably to fully supervised methods on all six applicable BOP core datasets, achieving within -11.3% to +0.2% of the top fully supervised results.

==> backup/backup-1/sec/0_abstract.tex <==
\begin{abstract}
We address the simulation-to-real domain gap in 
six degree-of-freedom pose estimation (6DoF PE), 
% ,
and propose a novel self-supervised keypoint voting-based 6DoF PE framework, effectively narrowing this gap using a learnable kernel in RKHS.
We formulate this domain gap as a distance in high-dimensional feature space,
distinct from previous iterative matching methods.
% We propose an adapter network,
% that evolves the network parameters from the source domain, which has been trained on synthetic data with synthetic poses, to the target domain, which is trained on real data.
We propose an adapter network,
which is pre-trained on purely synthetic data with synthetic ground truth poses,
and which evolves the network parameters
from this source synthetic domain to the target real domain.
Importantly, the real data training only uses pseudo-poses estimated by pseudo-keypoints, and thereby requires no real groundtruth data annotations.
Our proposed method is called
RKHSPose,
and achieves state-of-the-art performance 
among self-supervised methods
on three commonly used 6DoF PE datasets including LINEMOD ($+4.2\%$), Occlusion LINEMOD ($+2\%$), and YCB-Video ($+3\%$).
It also compares favorably to fully supervised methods 
on all six applicable BOP core datasets, %, which include
%LMO, YCB-V,
%T-LESS, TUD-L, ITODO, and HB.
achieving within $-11.3\%$
to $+0.2\%$ of the top fully supervised results.

\keywords{pose estimation \and self-supervision \and domain adaptation \and keypoint estimation}

\end{abstract}

==> backup/backup-1/sec/1_intro.tex <==
\section{Introduction}
\label{sec: Introduction}
% \begin{itemize}
%     \item 6dof pe problems
%     data hard to gather and label, some use syn ignoring syn/real gap, some requires multi models for multi instances/objects,
%     \item DA
%     various DA methods, DA in various other applications, some DA in 6d pose suffering (zzz,zzz,zzz)
%     \item propose a DA 6Dof pe method
%     single model, end-to-end, few-shot, robust
% \end{itemize}


RGB-D Six Degree-of-Freedom Pose Estimation (6DoF PE) 
is a problem being actively explored in Computer Vision (CV).
Given an RGB image 
% $I$ 
and its associated depth map, 
% $D$,
the task is to detect objects 
and estimate their poses comprising 
3DoF rotational angles and  3DoF translational offsets
in the camera reference frame.
This task enables many applications such as augmented reality~\cite{hinterstoisser2012model,posecnn,hodan2018bop,kaskman2019homebreweddb}, robotic bin picking~\cite{doumanoglou2016recovering,hodan2017tless,kleeberger2019large}, 
autonomous driving~\cite{ma2019accurate,xiao2019identity} and image-guided surgeries~\cite{gadwe2018real,greene2023dvpose}.
%[ zzz add one or two more ].

% Classical algorithms~\cite{hinterstoisser2012model} extract feature descriptors 
% to identify keypoints on the
% surface of the target object, 
% and estimate the pose
% by aligning these representations 
% from the CAD model to the segment in the image.

\input{figs/fig_teaser}

As with other machine learning (ML) tasks,
fully supervised
6DoF PE
requires large annotated datasets.
This requirement is particularly 
challenging
for 6DoF PE, as the annotations
comprise not only the identity of the objects
in the scene,
but also their 6DoF pose, which makes the data
relatively expensive to annotate
compared to related tasks such as
classification, detection and segmentation.
This is due to the fact that humans are not able to qualitatively or intuitively estimate 6DoF pose, which therefore requires additional instrumentation of the scene at data collection, and/or more sophisticated user annotation tools~\cite{hinterstoisser2012model, posecnn}.
% Initially, the classification task dataset was the most straightforward to label.
% It only requires one accurate classification label for each image,
% whereas datasets for object detection and semantic segmentation are relatively tricky.
% Labeling accurate bounding boxes and contours already takes more effort than assign a class label to an image.
% %Tasks such as classification, general object detection, and semantic segmentation take relatively less effort to label the data.
% The pose labels are even more ambiguous to be annotated, 
% especially on real 2D images.
% The bounding box and contour have a clear visual boundary 
% whereas the 6DoF pose of an object is not as intuitive as to be seen. 
Consequently,
synthetic 6DoF PE datasets~\cite{hodan2018bop,kleeberger2019large} have been introduced,
either as an additional complement to real datasets, or as standalone purely synthetic datasets.
Annotated synthetic datasets are of course trivially inexpensive to collect,
simply because
precise synthetic pose annotation
in a simulated environment is fully automatic.
A known challenge in using synthetic data, however, is that there typically exists a domain gap between the real and synthetic data, which makes results less accurate when 
inferring in real data using models trained on
purely synthetic datasets. 
Expectations of the potential benefit of synthetic datasets has led to the exploration of a rich set of Domain Adaptation (DA) methods, which specifically aim to reduce the domain gap~\cite{bozorgtabar2020exprada, zhang2017curriculum,pinheiro2019domain}
using inexpensive synthetic data
for a wide variety of tasks,
recently including 6DoF PE~\cite{guo2023knowledge,lee2022uda,li2021sd}.


%- mention that there exists a syn2real domain gap, i.e. synthetic images themselves are not as good on real images as real GT pose labels
%mentioned after the intuitive mixed syn real training 

Early methods~\cite{wu2022vote,kleeberger2020single} ignored the simulation-to-real (sim2real) domain gap and,
nevertheless improved performance by
training on both synthetic and real annotated data,
effectively augmenting the real images with the synthetic.
However, these methods still required real labels to be sufficiently accurate and robust for practical applications,
partially due to the domain gap.
As shown in Fig.~\ref{fig:teaser},
the rendered synthetic objects (left image) have a slightly different appearance than the real objects (right image).
The details of the CAD models, both geometry and texture, are not precise, as can be seen for the \emph{can} object (which lacks a mouth and shadows), the \emph{benchvise} (which is missing a handle), and the \emph{holepuncher} (which has coarse geometric resolution).
Several recent methods~\cite{kleeberger2021investigations,sundermeyer2018implicit,tan2023smoc,chen2023texpose,wang2020self6d} have
started to 
address the sim2real gap 
for 6DoF PE
by first training on labeled synthetic data 
and then fine-tuning on unlabeled real data.
These methods, commonly known as self-supervised methods,
reduce the domain gap
by adding extra supervision
using features extracted from real images without requiring real groundtruth (GT) labels.
The majority of these methods are viewpoint/template matching-based, and
the self-supervision commonly 
iteratively matches 2D masks or 3D point clouds~\cite{kleeberger2021investigations,sundermeyer2018implicit,wang2020self6d}.

While the above-mentioned self-supervison works have shown promise,
there exist a wealth of DA techniques that can be brought to bear to improve performance further for this task.
%[One such technique is zzz self-supervision, RKHS, etc.] 
One such technique is Reproducing Kernel Hilbert Space (\emph{RKHS}), which
is a kernel method that has been shown to be effective for DA~\cite{khosravi2023existence,al2021learning,bietti2019kernel}.
RKHS was initially used to create decision boundaries for non-separable data~\cite{cortes1995support,pearson1901liii},
and has
been shown to be effective at reducing the domain gap for various tasks and applications~\cite{zhang2018aligning,shan2023unsupervised,chen2020homm}.
The reproducing kernel guarantees that the domain gap can be statistically measured, allowing 
network parameters trained on synthetic data to be effectively adapted to the real data, using specifically tailored metrics.
%Although the domain gap between the synthetic and the real in 6DoF PE is moderate, this robust measurement can still be beneficial to narrow it better.
% RKHS is widely used in early ML techniques such as Support Vector Machines~\cite{cortes1995support} (SVMs) and Principle Component Analysis~\cite{pearson1901liii} (PCA). 
% These methods are commonly used for classification task in CV.
% The non-separable raw data becomes separable after being mapped into RKHS (increasing dimensionality).



%porting Domain Adaptation(zzz maybe Transfer Learning) techniques, 
%such as knowledge distillation~\cite{hinton2015distilling} and feature transfer~\cite{bozinovski1976influence},
% to match the features extracted from the viewpoint/template.
% Recent self-supervised methods
% have already demonstrated promising performance,
% approaching that of full supervision.

To address this sim2real domain gap in 6DoF PE, 
we propose RKHSPose,
which is a keypoint-based method~\cite{wu2022vote,wu2022keypoint} trained on a mixture of a large collection of labeled synthetic data, and a small handful of unlabeled real data.
% a Reproducing Kernel Hilbert Space (RKHS) based self-supervised 6DoF PE pipeline.
RKHSPose estimates
the intermediate radial voting quantity,
which has shown to be effective for estimating keypoints~\cite{wu2022vote},
by first training a modified FCN-Resnet-18
on purely synthetic data, with 
automatically labeled synthetic GT poses.
The radial quantity is a map of the distance from each image pixel to each keypoint.
Next, real images are passed through the synthetically trained network,
resulting in a set of pseudo-keypoints.
The real images and their corresponding pseudo-keypoints are used to render a
set of `synthetic-over-real' (\emph{synth/real}) images, by first estimating the pseudo-pose from the pseudo-keypoints, and then overlaying the synthetic object,
rendered with the pseudo-pose,
onto the real image. The network training
then continues on the synth/real images, invoking an RKHS network module with a trainable linear product kernel, which minimizes the Maximum Mean Discrepancy (MMD) loss. 
At the front end, a proposed 
keypoint radial voting network 
%(KRVNet) CNN
learns to cast votes to estimate keypoints
from the backend-generated radial maps.
The final pose is then determined using ePnP~\cite{lepetit2009ep} 
based on the estimated and corresponding object keypoints.

% An RKHS with a trainable linear product kernel 
% measured by Maximum Mean Discrepancy (MMD),
% is implemented
% during the self-supervision (fine-tuning) stage 
% on real unlabeled images.
% The RKHS network minimizes the domain gap between labels estimated 
% from synthetic pre-trained network on real images and pseudo labels on CAD model overlayed syn/real images.


The main contributions of this work are:
\begin{itemize}
    \item A novel learnable RKHS-based Adapter backend network architecture to minimize the sim2real domain gap in 6DoF PE;
    \item A novel CNN-based frontend network 
    %KRVNet
    %and a RANSAC style keypoint extraction 
    for keypoint radial voting;
    \item A self-supervised keypoint-based 6DoF PE method, RKHSPose, which is shown to have state-of-the-art (SOTA) performance, based on our experiments and several ablation studies. 
\end{itemize}


% Recent ML based~\cite{} methods tend to explore estimating the pose with a few/without 
% real GT labels simply due to the complexity of data gathering and labeling for 6DoF poses.
% These methods are often known as self-supervised methods as 
% a template overlay state is typically included

==> backup/backup-1/sec/2_background.tex <==
\section{Related Work}
\label{sec: Related Works}
\subsection{6DoF PE}
\input{tabs/tab_6d_info_missing_methods}
ML-based 6DoF PE methods~\cite{posecnn,oberweger2018making,pvnet} 
all train a network to 
regress quantities,
such as 
keypoints and camera viewpoints,
as have been used in classical algorithms~\cite{hinterstoisser2012model}.
ML-based methods,
which
initially became popular for the general object detection task,
have started to dominate the 6DoF PE literature
due to their accuracy and efficiency.

There are two main categories of ML-based fully supervised methods:
\emph{feature matching}-based~\cite{posecnn,oberweger2018making,su2022zebrapose,haugaard2022surfemb,hai2023rigidity}, and 
\emph{keypoint}-based methods~\cite{pvnet,pvn3d,he2021ffb6d,yang2023object}.
% Feature matching-based methods 
% are
% the most intuitive conversion of
% a trainable network from 
% general object detection frameworks.
Feature matching-based methods
make use of the structures from
general object detection networks
most directly.
The network encodes and matches features and estimates pose
by either regressing elements of the pose
(e.g. the transformation matrix~\cite{tan2023smoc}, rotational angles and translational offsets~\cite{posecnn} or 3D vertices~\cite{su2022zebrapose}) directly,
or 
by regressing some intermediate feature-matching representations, such as viewpoints or segments.

In contrast, 
keypoint-based methods encode features
to estimate keypoints 
which are predefined
within the reference frame of an object's CAD model.
These methods then use (modified) classical algorithms
such as PnP~\cite{p3p,lepetit2009ep}, Horn's method~\cite{horn1988closed}, 
and ICP~\cite{besl1992icp}
to estimate the final pose
from corresponding image and model keypoints. 
Unlike feature-matching methods,
keypoint-based methods are typically more accurate due to
redundancies encountered 
through voting schemes~\cite{pvnet,wu2022vote,pvn3d} 
and by generating confidence hypotheses of keypoints~\cite{he2021ffb6d,yang2023object}.
% \begin{itemize}
%     \item supervised
%             issues: hard to capture gt info
%             Knowledge Distillation for 6D Pose Estimation
% by Aligning Distributions of Local Predictions

%     \item semi/unsupervised
%     \cite{tan2023smoc}
%         \cite{zhou2023deep}- least square linear voting
%         Sim2Real Instance-Level Style Transfer for 6D Pose Estimation
%         Sim-to-Real 6D Object Pose Estimation via
% Iterative Self-training for Robotic Bin Picking
% \end{itemize}

%LatentFusion~\cite{park2020latentfusion}  latent modeling, rendering, pose by predict depth
%FS6D~\cite{he2022fs6d} transformer based, render texture on texture less obj, PC image fusion
%OSOP~\cite{shugurov2022osop} sparse viewpoint, dense matching fine-tune(template, 2d mask),
 %Xiao \etal~\cite{xiao2019pose} data aug, test on unseen
%Sundermeyer~\cite{sundermeyer2020multi} PCA encoding codebook, iterative matching
%Kleeberger \etal~\cite{kleeberger2021investigations} add noise to training
%Su \etal~\cite{su2015render}viewpoint, render model on real bg
%Self6D~\cite{wang2020self6d} and slef6d++~\cite{wang2021occlusion} render and align, visual(2d mask) and geometry (pc)
%Deng \etal~\cite{deng2020self} iteratively match
%TexPose~\cite{chen2023texpose} matching cad model to nerf generated segment
%MOC-Net~\cite{tan2023smoc} use structure from motion
%DPODv2~\cite{shugurov2021dpodv2} texture render, dense correspondence

%AAE~\cite{sundermeyer2018implicit} DA by codebook
%MHP~\cite{Manhardt_2019_ICCV} symmetric Bingham distributions
%Sock \etal~\cite{sock2020introducing} render syn imgs using differentiable pnp~\cite{chen2020end} and render~\cite{kato2018neural}
%DSC~\cite{xiao2019pose} scale consistency by differentiable pnp and renderer
% Despite fully-supervised methods, 
Recently, self-supervised 6DoF PE methods have been explored in order to reduce the reliance on labeled real data,
which is expensive to acquire.
As summarized in Table~\ref{tab:self supervised 6DoF PE}, these methods commonly use real images without GT labels.
Some methods use pure synthetic data and CAD models only, with the exception of LatentFusion~\cite{park2020latentfusion} which trained the model using only synthetic data.
The majority of these methods~\cite{he2022fs6d,shugurov2022osop,sundermeyer2020multi,su2015render,wang2020self6d,deng2020self,wang2021occlusion,chen2023texpose,tan2023smoc,sock2020introducing, lin2022category}
are inspired by fully supervised feature-matching methods, except DPODv2~\cite{shugurov2021dpodv2} and DSC~\cite{xiao2019pose}, in which keypoint correspondences are
rendered and matched.

A few methods~\cite{shugurov2022osop,deng2020self}
%and Deng \etal~\cite{deng2020self} 
fine-tuned the pose trivially by iteratively matching the template/viewpoint, whereas
others~\cite{xiao2019pose,kleeberger2021investigations,park2020latentfusion,he2022fs6d} augmented the training data by adding noise~\cite{xiao2019pose,kleeberger2021investigations}, rendering textures~\cite{he2022fs6d,shugurov2021dpodv2} and
creating a latent space~\cite{park2020latentfusion}.
% others~\cite{xiao2019pose,kleeberger2021investigations,park2020latentfusion,he2022fs6d} augmented the training data by adding noises~\cite{xiao2019pose,kleeberger2021investigations}, rendering textures~\cite{he2022fs6d,shugurov2021dpodv2} and
% creating a latent space~\cite{park2020latentfusion}.
Some methods~\cite{sundermeyer2018implicit,sundermeyer2020multi,Manhardt_2019_ICCV} also implemented DA techniques such as encoding a codebook~\cite{sundermeyer2020multi}, Principle Component Analysis (PCA)~\cite{sundermeyer2020multi} and symmetric Bingham distributions~\cite{Manhardt_2019_ICCV}.
Most methods~\cite{shugurov2022osop,su2015render,wang2020self6d,wang2021occlusion,sock2020introducing,xiao2019pose} used rendering techniques to render and match a template.
There are a few methods that combined  3D reconstruction techniques, such as Neural radiance fields (Nerf)~\cite{mildenhall2021nerf} and Structure from Motion (SfM)~\cite{ullman1979interpretation}.
TexPose~\cite{chen2023texpose} matched CAD models to segments generated by Nerf,
and SMOC-Net~\cite{tan2023smoc} used SfM to create the 3D segment and matched with the CAD model.


\subsection{Kernel Methods and Deep Learning}
While Deep Learning (DL) is the most common ML technique within the CV literature,
kernel methods~\cite{cortes1995support,pearson1901liii,sejdinovic2013equivalence} have also been actively  explored.
Kernel methods are typically in RKHS space~\cite{szafraniec2000reproducing} with reproducing properties that facilitate solving
non-linear problems by
mapping input data into high dimensional spaces where they can be linearly separated~\cite{ghojogh2021reproducing,corcoran2020end}.
Well-known early kernel methods that have been applied to CV are Support Vector Machines~\cite{cortes1995support} (SVMs) and PCA~\cite{pearson1901liii}. 
A recent method~\cite{sejdinovic2013equivalence} linked energy distance and MMD in RKHS, 
and showed the effectiveness of kernels in statistical hypothesis testing. 

More recent studies compare kernel methods with DL networks~\cite{khosravi2023existence,al2021learning,bietti2019kernel,bietti2019group}.
RKHS is found to 
 perform better on classification tasks 
than one single block of a CNN comprising convolution, pooling and downsampling (linear) layers~\cite{khosravi2023existence}. 
RKHS can also help with CNN generalization by meta-regularization on image registration problems\cite{al2021learning}.
Similarly, norms (magnitude of trainable weights) defined in RKHS help with  CNN regularization~\cite{bietti2019kernel,bietti2019group}.
%based on their previous stability analysis~\cite{bietti2019group}.
Further, discriminant information in label distributions in unsupervised DA is addressed and RKHS-based Conditional Kernel Bures metric is proposed~\cite{luo2021conditional}.
Lastly, the connection between Neural Tangent Kernel and MMD is established,
and an efficient MMD for two-sample tests is developed~\cite{cheng2021neural}.

%Extending from 
Inspired by the previous work,
RKHSPose applies concepts of kernel learning to keypoint-based 6DoF PE,
to provide an effective means to self-supervise a synthetically trained network on unlabeled real data.


==> backup/backup-1/sec/3_method.tex <==
\section{Method}
\label{sec:Method}
\input{figs/fig_diagram}
\subsection{Network Overview}
\begin{comment}
    

\begin{itemize}
    \item main model M, trained mainly on syn with a few real samples. 
    \item The Adapter A functions as an additional supervision for training.
\end{itemize}
\begin{itemize}
          \item Network Structure 
          Main Model
            Input: RGB and Standardized D
            Output: Radii Map, projected kpts, class+confidence score, intermediate feature maps
            Loss:Corss entropy for classification, smoothl1 for kpt location and radii map
          Adapter
            Input: feature maps pairs from Syn and Real training
            Output: Similarity score 
            Loss: MMD within RKHS
           \item Training Strategy 
           Train mainly with syn, and reals are trained during the syn training with a fixed interval limited by time and sample of images.
           Adapter A steps in right after each real epoch, calculates gradients for both Main model M and D.
           \item GPU voting
           In order to vote for keypoints, instead of using voxel space voting ~\cite{wu2022vote,pvnet,pvn3d,wu2022keypoint}, 
           follow votenet ~\cite{qi2019deep},
           accumulate votes by casting radii into conv layers
           loss is the normalized radial distances from gt points to estimated points.
           \item RANSAC voting (zzz)
           
\end{itemize}
\end{comment}

As shown in Fig.~\ref{fig:diagram}, RKHSPose is made up of two networks,
one main network $M_{rv}$ for keypoint regression and classification, 
and one Adapter network $M_A$. 
% to minimize the synthetic-real domain gap
% by densely comparing the feature maps of 
% every convolution block of $M_{rv}$ trained on both synthetic and real images.  
The input of $M_{rv}$ 
with shape $W\!\times\!H\!\times\!4$, 
is the concatenation of an RGB image $I$ and its corresponding depth map $D$.
This input can be synthetically generated with an arbitrary background ($I_{syn}$ and $D_{syn}$),
a synthetic mask overlayed on a real background ($I_{syn/real}$ and $D_{syn/real}$),
or real ($I_{real}$ and $D_{real}$) images.
The outputs are $n$ projected 2D keypoints $K$, 
along with corresponding classification labels $C$ and confidence scores $S$. $K$ are organized into instance sets based on $C$ and geometric constraints.

$M_{rv}$ comprises two sub-networks, 
% voting quantity 
regression network $M_r$ and % probability 
voting network $M_v$.
Inspired by recent voting techniques~\cite{pvnet,pvn3d,wu2022vote,wu2022keypoint,zhou2023deep},
$M_r$ estimates an intermediate voting quantity, 
which is a radial distance map $V_r$~\cite{wu2022vote}, 
by using a modified Fully Connected ResNet 18 (FCN-ResNet-18).
The radial voting map $V_r$, with shape $W\!\times\!H$,
stores the Euclidean distance
from each object point to each keypoint
in the 3D camera world reference frame.
The voting network $M_v$ 
(described in Sec.~\ref{sec: Keypoints ConvRVoting})
then takes $V_r$ as input, 
accumulates votes, and detects the peak to
estimate $K$, $C$ and $S$.


The Adapter network $M_A$ consists of
a series of CNNs 
which encode pairs of feature maps from $M_{rv}$,
and are trained on both synthetic overlayed and pure real data.
$M_A$ encodes
feature map pairs $(f_{syn/real}, f_{real})$ 
into corresponding high-dimensional feature maps $(h_{syn/real}, h_{real})$.
The input data, 
$(I_{syn/real},I_{real})$ and $(D_{syn/real},D_{real})$,
are also treated as $(f_{syn/real}, f_{real})$ during the learning of $M_A$.
Each of these networks creates a high-dimensional latent space,
essentially the Reproducing Kernel Hilbert Space (RKHS)~\cite{aronszajn1950theory}
and contributes to the learning of both $M_{rv}$ and $M_A$ 
by calculating the 
%Maximum Mean Discrepancy 
MMD~\cite{gretton2012kernel}.
While RKHS has been applied effectively to other DA tasks, to our knowledge, this is the first time that it has been applied to 6DoF PE, and the adapter network architecture is novel.

The loss function $\mathcal{L}$ is made up of five elements:
Radial regression loss $\mathcal{L}_{r}$ for $V_r$;
Keypoint projection loss $\mathcal{L}_{k}$ for $K$;
Classification loss $\mathcal{L}_{c}$ for $C$; 
Confidence loss $\mathcal{L}_{s}$ for $S$, and finally;
Adapter loss $\mathcal{L}_{M_A}$ for the comparison of intermediate feature maps.
% The regression losses $\mathcal{L}_{r}$, $\mathcal{L}_{k}$, and $\mathcal{L}_{s}$ all use the smooth L1 metric, whereas classification loss $\mathcal{L}_{c}$ uses the cross-entropy metric.
The regression losses $\mathcal{L}_{r}$, $\mathcal{L}_{k}$, and $\mathcal{L}_{s}$ all use the smooth L1 metric, whereas classification loss $\mathcal{L}_{c}$ uses the cross-entropy metric $H(\cdot)$.
RKHSPose losses can then be denoted as:
% \begin{equation}
%     \mathcal{L}_{r} = smooth_{\mathcal{L}_1}(\widehat{V_r},V_r)
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{k} = smooth_{\mathcal{L}_1}(\widehat{K},K)
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{c} = H(p(C), \widehat{p(C)})
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{s} = smooth_{\mathcal{L}_1}(\widehat{S},S)
% \end{equation}
% \begin{equation}
%     \mathcal{L}_{M_A} = MMD(\widehat{f_{syn/real}}, \widehat{f_{real}})
% \end{equation}
% % \begin{equation} 
% %     \mathcal{L} = \lambda_r  \mathcal{L}_{r} + \lambda_k \mathcal{L}_{k} + \lambda_c  \mathcal{L}_{c} + \lambda_r  \mathcal{L}_{s} + \lambda_D \mathcal{L}_{M_A}
% % \end{equation}
% \begin{equation} 
%     \mathcal{L} = \lambda_r \mathcal{L}_{r} + \lambda_k \mathcal{L}_{k} + \lambda_c \mathcal{L}_{c} + \lambda_s \mathcal{L}_{s} + \lambda_D \mathcal{L}_{M_A}
% \end{equation}
\begin{eqnarray}
% \begin{equation}
\mathcal{L}_{r} 
&=& 
% =
smooth_{\mathcal{L}_1}(V_r, \widehat{V_r})
% \end{equation}
% \begin{eqnarray}
\\
\mathcal{L}_{k} &=& smooth_{\mathcal{L}_1}(K, \widehat{K})
\\
\mathcal{L}_{c} &=& H(p(C), \widehat{p(C)})
\\
\mathcal{L}_{s} &=& smooth_{\mathcal{L}_1}(S, \widehat{S})
% \end{eqnarray}
% \begin{eqnarray}
\\
\mathcal{L}_{M_A} &=& MMD(\widehat{f_{syn/real}}, \widehat{f_{real}})
\\
\mathcal{L} = \lambda_r \mathcal{L}_{r}
&+&
\lambda_k \mathcal{L}_{k} + \lambda_c \mathcal{L}_{c} + \lambda_s \mathcal{L}_{s} + \lambda_D \mathcal{L}_{M_A}
\end{eqnarray}
% \begin{equation}
% \mathcal{L} = \lambda_r \mathcal{L}_{r} + \lambda_k \mathcal{L}_{k} + \lambda_c \mathcal{L}_{c} + \lambda_s \mathcal{L}_{s} + \lambda_D \mathcal{L}_{M_A}
% \end{equation}
\noindent where
$\lambda_r$, $\lambda_k$, $\lambda_c$, $\lambda_s$, and $\lambda_D$ are weights for adjustment during training,
and all non-hatted quantities are GT values. 
At inference, $M_{rv}$ takes the $I_{real}$ and $D_{real}$ as input, and
 outputs  $K$, $C$ and $S$.
The keypoints $K$ are ranked and grouped by $S$ and $C$, and are then forwarded into the ePnP~\cite{lepetit2009ep} algorithm which estimates 6DoF pose values. 

\subsection{Convolutional RKHS Adapter}
\label{sec: Convolutional RKHS Discriminator}
\begin{comment}
    

\begin{itemize}
    \item rkhs
    Two sets of data (such as feature maps produced by pretrained synthetic and real weights), 
    RKHS defines a reproducing hilbert space (two linear functions $h(x_{syn})$, $g(x_{real})$) to represent the discrete data points, 
    if $\|h(x_{syn})-g(x_{real})\|$ are close in RKHS, all data points of $x_{syn}$ and $x_{real}$ should also be close~\cite{berlinet2011reproducing,drewnik2021reproducing,misiakiewicz2022learning}.

    % Not sure if needed, but define RKHS
    Let $X$ be a set of data whose dimension can be infinite and 
    $H$ be a Hilbert space represented by Euclidean vectors with finite dimension,
    $H$ is an RKHS if an evaluation function $L_x$ within $H$ exists for each function $g(x)$ at a point $x$ within $X$~\cite{berlinet2011reproducing}.
    It can be denoted as:
    \begin{equation}
        L_x: g \mapsto g(x) \forall g \in H .
    \end{equation}
    In order to define $L_x$, the most intuitive way is an inner product function $K_x$ of $g$~\cite{zzz}. 
    If $y$ is another set of data, $K_y$ should also exist, 
    the reproducing kernel can then defined as:
    \begin{equation}
        K(x, y)=\left\langle K_x, K_y\right\rangle_H
    \end{equation}

    These definitions are also true for feature maps.
    A feature map $\varphi$ can be the output of the conv layer within Model M, the feature maps trained on syn and real can be denoted as $\varphi(x_{syn})$ and $\varphi(x_{real})$. The RKHS kernel can then be:
    \begin{equation}
        K(x, y)=\langle\varphi(x_{syn}), \varphi(x_{real})\rangle_{H\cdot}
    \end{equation}
    where K is the kernel and H is the Hilbert space.
    The similarity of feature maps can then be measured by the maximum mean discrepancy (MMD), which is the square distance between the embedding $K$.
    
    \item rkhs with conv
     On one hand,$\varphi(x_{syn})$ and $\varphi(x_{real})$ can be directly matched by MMD applying a inner product within RKHS
     On the other hand, RKHS works better when the raw data(feature map) spaces are infinite.
     The direct dense matching already extended the dimension of feature spaces, however, 
     it is still relatively restricted by the training data,
     whether synthetic or real,
     In order to further extend the dimension of feature spaces,
     conv layers are applied to each of feature maps and 
     MMD is measured on the output of these conv layers, shown in fig.~\ref{fig:zzz}.
     Extra conv layers simulate the infinite dimension feature space between syn and real (impact of ambient, occlusion, camera sensor), 
     forms our Adapter A, making the domain adaptation more robust.
     
\end{itemize}
\end{comment}
% Bridging the domain gap between real and synthetic data for the 6DoF PE problem
% has been recently addressed by~\cite{chen2023texpose,wang2021gdr,Di_2021_ICCV}.
% Motivated by these methods, 
% the main objective of RKHSPose is to
% minimize this gap so that 
% PE can be accomplished with
% only a few real samples.
\begin{comment}
%f->conv
%K->MMD
%L->smoothl1
zzz - maybe move or remove this paragraph:

START

Instead of using classical RKHS~\cite{zhou2021semi},
a deep RKHS-based Adapter $M_A$ is introduced to synchronize the mixed synthetic-real training. 

END

% With two sets of data $X$ and $Y$,
% RKHS denotes a reproducing Hilbert space
% where two linear functions, $h(x)$ and $g(y)$, are used to represent the data.
% The distance between $x$ and $y$ should be close ($\left|h(x)-g(y)\right|$ is small for all $x$ and $y$)
% when $\|h(x)-g(y)\|$ is small in RKHS.

zzz - add high level description of Hilbert space and RKHS. Why is it important, what does it do, why do we care?

With two sets of data $X$ and $Y$,
RKHS denotes a reproducing Hilbert space,
where functions $h(x)$ and $g(y)$ are used to represent the data.
These two functions are linear,
and 
%compress their possibly different, low-dimensional input data into a common
 map all $x\!\!\in\!\!X$ and $y\!\!\in\!\!Y$ 
into Hilbert space.
%Once mapped,
If the distance between
$h$ and $g$
is small,
then
$h(x)$ and $g(y)$
are close, i.e.:

%zzz check for accuracy, and replace with correct version
zzz revised, think it is correct
\begin{equation}
    \|h-g\|
    \rightarrow
    |h(x)-g(y)| \le \epsilon
\end{equation}
The utility of mapping into Hilbert space is 
that similarity in Hilbert space serves as a proxy for similarity in the original %higher dimensional
immeasurable data,
and so it provides an effective means to compare data, e.g. kernel methods using MMD. 

Specifically, 
let $X$ be a set of data whose inseparable in lower dimension spaces, and 
let $H$ be a high dimension inner product Hilbert space represented by Euclidean vectors.
$H$ is 
%considered as
an RKHS (a complete inner product space with reproducing property) if
a linear evaluation function $L_x$ within $H$ exists (is continuous)
for each function $g(x)$
from a set of functions $g$,
for all points $x \in X$~\cite{berlinet2011reproducing}, i.e.:
\begin{equation}
    L_x:g\mapsto g(x) \; \forall \; g \in H .
\label{eq:rkhs}
\end{equation}
This guarantees that $L_x$ evaluates all functions $g$ of $X$, despite it being 
hard in general to explicitly define the boundary function $L_x$~\cite{zzz}.
An intuitive way to approximate $L_x$
is through
the reproducing kernel function $K_x$, which is the inner product of $g$. 
Based on the Riesz representation theorem~\cite{zzz}, 
a unique $K_x$ of $H$ exists for $X$ with the reproducing property, which is expressed as:
\begin{equation}
    g(x) = L_x(g) = \left\langle g, K_x\right\rangle_H\; \forall \; g \in H .
\end{equation}
where $\left\langle a, b\right\rangle$ is the inner product of a and b.
\end{comment}
%add high level description of Hilbert space and RKHS. Why is it important, what does it do, why do we care?
Reproducing Kernel Hilbert Space $\mathcal{H}$ is a commonly used vector space for Domain Adaptation~\cite{pan2010domain,venkateswara2017deep}.
% It is a Hilbert Space with a reproducing kernel.
Hilbert Space is a complete metric space 
(in which every Cauchy sequence of points has a limit within the metric) 
represented by the inner product of vectors.
For a non-empty set of data $\mathcal{X}$,
a function $K_X\!:\!\mathcal{X}\!\times\!\mathcal{X}\!\rightarrow\!\mathcal{R}$ is a reproducing kernel if:
% \begin{itemize}[leftmargin=2.0cm]
%     \item $\forall x \in \mathcal{X}, k(\cdot,x) \in \mathcal{H}$
%     \item $\forall x \in \mathcal{X}, \forall f \in \mathcal{H}, \left\langle f(\cdot), k(\cdot,x)\right\rangle = f(x)$
% \end{itemize}
%
\begin{equation}
\begin{cases}
    &k(\cdot,x) \in \mathcal{H}\;\;\; \forall \;\;\; x \in \mathcal{X} \\
    & \left\langle f(\cdot), k(\cdot,x)\right\rangle = f(x) \;\;\; \forall \;\;\; x \in \mathcal{X}, f \in \mathcal{H}
\end{cases}
\label{eq:cases}
\end{equation}
%
where $\left\langle a, b \right\rangle$
denotes the inner product of two
vectors $a$ and $b$,
$k(\cdot,x)=K_\mathcal{X}$ 
for each $x\!\in\!\mathcal{X}$, 
and $f$ is a function in $\mathcal{H}$.
The second equation in
Eq.~\ref{eq:cases}
is an expression of the reproducing property of $\mathcal{H}$.

In order to utilize $\mathcal{H}$ for DA,
we expand the kernel definition to 
two sets of data $\mathcal{X}$ and $\mathcal{Y}$.
The reproducing kernel
 can then be defined as:
% If $y$ is another set of data, then $K_y$ should also exist, and
% the reproducing kernel of $x$ and $y$ can then be defined as:
\begin{equation}
    K(\mathcal{X}, \mathcal{Y})=\left\langle K_\mathcal{X}, K_\mathcal{Y}\right\rangle_H
\label{eq:rkhs_k}
\end{equation}
Here, 
$K_\mathcal{X}$ and $K_\mathcal{Y}$ are 
themselves inner product kernels
that map $\mathcal{X}$ and $\mathcal{Y}$ respectively into their own Hilbert spaces,
and 
% $\langle K_X,K_Y\rangle_H$ 
$ K(\mathcal{X}, \mathcal{Y})$
is the joint Hilbert space kernel
of $\mathcal{X}$ and $\mathcal{Y}$.
Note that $ K(\mathcal{X}, \mathcal{Y})$ is not the kernel commonly defined for CNNs. 
Rather, it is the similarity function defined in kernel methods, such as is used by SVM techniques to calculate similarity measurements.
Some recent methods~\cite{misiakiewicz2022learning,mairal2014convolutional,mairal2016end,chen2020convolutional} named it a Convolutional Kernel Network (CKN) in order to distinguish it from CNNs.

Various kernels of CKN, such as 
the Gaussian Kernel~\cite{mairal2014convolutional}, the RBF Kernel~\cite{mairal2016end} and the Inner Product Kernel~\cite{misiakiewicz2022learning}, 
have been shown to be comparable to shallow CNNs for various tasks, especially for Domain Adaption.
The most intuitive inner product kernel 
% $K$ 
% defined in Eq.~\ref{eq:rkhs_k} 
is mathematically similar to 
a fully connected layer, 
where trainable weights are multiplied by the input feature map.
To allow the application of RKHS methods into our CNN based Adapter network $M_A$, 
% and RKHS interact with a shared layer/kernel,
trainable weights are added to $K(\mathcal{X}, \mathcal{Y})$~\cite{liu2020learning}.
% inspired by FC layer.
The trainable Kernel $K_{w}(\mathcal{X}, \mathcal{Y})$ can then be denoted as:
\begin{equation}
    K_{w}(\mathcal{X}, \mathcal{Y}) = \left \langle \left\langle \mathcal{X},W_\mathcal{X}\right\rangle,\left\langle \mathcal{Y},W_\mathcal{Y}\right\rangle \right\rangle_H
\label{eq:kw}
\end{equation}
where $W_\mathcal{X}$ and $W_\mathcal{Y}$ are trainable weights. 
By adding $W_\mathcal{X}$ and $W_\mathcal{Y}$ , $K_{w}(\mathcal{X}, \mathcal{Y})$
still satisfies the
%the two
RKHS constraints.
%of RKHS.
%reproducing property, 
%and is in an expanded RKHS $\mathcal{H}$.

%Considering $f_{syn}$ and $f_{real}$, 
% These definitions are also true~\cite{bietti2019kernel} if the data is a matrix such as 
%$I$, $D$, and 
%Considering $f$ in our model $M_{rv}$ and $M_A$,
%an RGB image, a depth map, or a feature map of a convolution layer.
The sim2real domain gap of feature maps $f$ being trained in $M_{rv}$ (with few real images and no real GT labels)
are hard to measure using trivial distance metrics.
%   which makes
% On the other hand, 
% a simple direct comparison, between synthetic and real training 
% measuring either topological or Euclidean distance, 
% can lead the training towards local minim.
%would be too narrow for 
% $M_{rv}$ less robust at inference.
In contrast, RKHS can be a more accurate and robust space for comparison, since
it is known to be capable of handling high-dimensional data with a low number of samples~\cite{ghorbani2020neural,misiakiewicz2022learning}.
To compare $(f_{syn/real}, f_{real})$ in RKHS,
a series of CNN layers encodes $(f_{syn/real}, f_{real})$ into higher-dimensional features $(h_{syn/real}, h_{real})$,
followed by the trainable $K_w(\mathcal{X}, \mathcal{Y})$.
%The RKHS kernel can then be denoted as:
% \begin{equation}
%     K(h_{syn/real},h_{real})=\langle g(h_{syn/real}), g(h_{real})\rangle_{H\cdot}
% \label{eq:rkhs_k_f}
% \end{equation}
%where $g()$ is the kernel function, K is the kernel and H is the Hilbert space.
Once mapped into RKHS, 
%$h_{syn/real}\! = \!\{sr_i|sr_i \in h_{syn/real}, i=0,1,...,m\}$
$h_{syn/real}\! = \!\{sr_i\}_{i=1}^{m}$
%   $, i=0,1,...,m-1$
and 
%$h_{real}\! = \!\{r_j|r_j \in h_{real}, j=0,1,...,m\}$ 
$h_{real}\! = \!\{r_i\}_{i=1}^{m}$
%   with a length of $M_{rv}$ 
can then be measured by Maximum Mean Discrepancy (MMD), a common DA measurement~\cite{gretton2012kernel,liu2020learning}, which is the square distance between the kernel embedding~\cite{gretton2006kernel}:
\vspace{-\baselineskip}
% \begin{equation}
% \begin{split}
%     MMD(h_{syn/real},h_{real}) =  
%         &
%     (\frac{1}{m^2}(\sum_{i,j=0}^{m-1,m-1}{k_w(sr_i,sr_j)} - \\& \sum_{i,j=0}^{m-1,m-1}{k_w(sr_i,r_j)} +\\
%     &\sum_{i,j=0}^{m-1,m-1}{k_w(r_i,r_j)} ))^{0.5}
% \end{split}
% \label{eq:mmd}
% \end{equation}

% \begin{equation}
% \begin{split}
% MMD(h_{syn/real},h_{real}) = 
%    \left(\frac{1}{m^2} \left( 
% \left(\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}{k_w(sr_i,sr_j)} \right.\right. \right.
% \\- 
% \left.\sum_{i=0}^{m-1}{k_w(sr_i,sr_i)}\right)
% \\
% - \left(\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}{k_w(sr_i,r_j)} \right.
% \\- 
% \left.\sum_{i=0}^{m-1}{k_w(sr_i,r_i)}\right)
% \\+\left(\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}{k_w(r_i,r_j)}\right.\\
% - \left.\left.\left.\sum_{i=0}^{m-1}{k_w(r_i,r_i)}\right)\right)\right)^{0.5}
% \end{split}
% \label{eq:mmd2}
% \end{equation}
%
% \begin{eqnarray}
% % \begin{split}
% MMD(h_{syn/real}, h_{real}) = \hspace{4 cm} \\
% \left[\frac{1}{m^2} \left( 
% \left(\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}{k_w(sr_i,sr_j)}\right.\right.\right.
% - 
% \left.\sum_{i=0}^{m-1}{k_w(sr_i,sr_i)}\right)
% \nonumber \\
% -\left(\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}{k_w(sr_i,r_j)} \right.
% - 
% \left.\sum_{i=0}^{m-1}{k_w(sr_i,r_i)}\right)
% \nonumber \\
% +\left(\sum_{i=0}^{m-1}\sum_{j=0}^{m-1}{k_w(r_i,r_j)}\right.
% - \left.\left.\left.\sum_{i=0}^{m-1}{k_w(r_i,r_i)}\right)\right)\right]^{0.5}
% \nonumber
% % \end{split}
% \label{eq:mmd2}
% \end{eqnarray}
%
% \begin{comment}
% \begin{align}
% % \begin{split}
% MMD(&h_{syn/real}, h_{real}) = \hspace{3 cm} \\
% \left[\frac{1}{m^2} \right.
% &\left( 
% \left(\sum_{i=1}^{m}\sum_{j=1}^{m}{k_w(sr_i,sr_j)}\right.\right.
% - 
% \left.\sum_{i=1}^{m}{k_w(sr_i,sr_i)}\right)
% \nonumber \\
% &-\left(\sum_{i=1}^{m}\sum_{j=1}^{m}{k_w(sr_i,r_j)} \right.
% - 
% \left.\sum_{i=1}^{m}{k_w(sr_i,r_i)}\right)
% \nonumber \\
% &+\left(\sum_{i=1}^{m}\sum_{j=1}^{m}{k_w(r_i,r_j)}\right.
% - \left.\left.\left.\sum_{i=1}^{m}{k_w(r_i,r_i)}\right)\right)\right]^{0.5}
% \nonumber
% % \end{split}
% \label{eq:mmd2}
% \end{align}
% \end{comment}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
% \begin{split}
MMD(h_{syn/real}, h_{real}) =
\left[\frac{1}{m^2}\right.
&\left(\left(\sum_{i=1}^{m}\sum_{j=1}^{m}{k_w(sr_i,sr_j)}\right.\right.
- 
\left.\sum_{i=1}^{m}{k_w(sr_i,sr_i)}\right)
% \\
\nonumber \\
&-\left(\sum_{i=1}^{m}\sum_{j=1}^{m}{k_w(sr_i,r_j)} \right.
- 
\left.\sum_{i=1}^{m}{k_w(sr_i,r_i)}\right)
\\
% \nonumber \\
&+\left(\sum_{i=1}^{m}\sum_{j=1}^{m}{k_w(r_i,r_j)}\right.
- \left.\left.\left.\sum_{i=1}^{m}{k_w(r_i,r_i)}\right)\right)\right]^{0.5}
\nonumber
% \end{split}
\label{eq:mmd2}
\end{align}

where $k_w()$ is the feature element of $K_w()$.


% Further, recent studies combining Convolution Neural Networks (CNN) with RKHS~\cite{ghojogh2021reproducing,drewnik2021reproducing,bertsimas2022data,zhou2021semi,bietti2019kernel} 
% shows that RKHS can improve the training of CNN in various aspects.
% The convolution operation and the gradient descent mchanism can simulate RKHS by projecting raw data into separable latent spaces.

In summary, the Adapter $M_A$, shown in Fig.~\ref{fig:diagram}, 
measures MMD 
for each $(h_{syn/real}, h_{real})$ in RKHS 
by increasing the $f_{syn/real}$ and $f_{real}$ dimension using a CNN and 
thereby constructing a learnable kernel $K_w$.
The outputs are the 
feature maps
$h_{syn/real}$ and $h_{real}$ 
which are supervised by loss
 $\mathcal{L}_{M_A}$, 
during training of the real data epochs.
Based on the experiments in Sec.~\ref{sec: Discriminator Kernels Metrics},
our trainable inner product kernel is
shown to be more accurate
for our task
than other known kernels~\cite{mairal2014convolutional,mairal2016end,misiakiewicz2022learning} that we tested, that are used in such kernel methods.


\subsection{Keypoint Radial Voting Network}
\label{sec: Keypoints ConvRVoting}
\begin{comment}
    

\begin{itemize}
    \item GPU Voting
    recap of different votes on GPU: PVNet and votenet vote on vector/offset fully paralleled on GPU combined with a confidence score estimated by the CNN, 
    radial voting on GPU: 
    rcvpose proposed radial, a more accurate, relatively more expensive voting for keypoints.
    Given a 2D radii map $V_r$, object pixels store radial distance to keypoints, background pixels are -1, task is to accumulate votes to estimate the keypoint location.
    instead of voxel voting,  create a 2D voxel space and render circles,
    use an MLP $M_v$ to vote, the MLP takes $V_r$ and generates heat map, the heat map is then reshaped to $n \times 4$ output by a fully connected layer. The output is $(K_n, C_n, S_n)$. 
    $M_v$ trained with $M_r$ supervised by $\mathcal{L}_k$, $\mathcal{L}_C$, and $\mathcal{L}_S$.
    
    \item RANSAC Voting
\end{itemize}

\end{comment}
% \input{figs/fig_v_r}
The network $M_v$ votes for keypoints using a CNN architecture, taking the radial voting quantity
$V_r$
resulting from $M_r$
as input.
VoteNet~\cite{qi2019deep} previously used a CNN approach to vote for object centers,
whereas other keypoint-based techniques have implemented
GPU-based
parallel RANSAC~\cite{pvn3d,pvnet} methods for offset and vector quantities.
The radial quantity is known to be more accurate but less efficient than the vector or offset quantities, and 
has been previously implemented with a CPU-based
parallel 
accumulator space method~\cite{wu2022vote,wu2022keypoint}.
% Recent work has shown that
% GPU voting is robust and efficient (enabling end-to-end training and testing)
% when voting on the
% vector~\cite{pvnet} and offset~\cite{pvn3d,qi2019deep}
% quantities.
%Existing radial voting methods~\cite{wu2022vote,wu2022keypoint} have used classical voting which is either analytical or voxel-based.
% Although radial voting is more accurate than offset or vector, it has also been relatively less efficient.

Given its superior accuracy, 
$M_v$ implements radial voting using a CNN to
improve efficiency.
% The voting is parallelized on a GPU, 
% and jointly estimates confidence scores alongside the radial votes themselves, thereby improving robustness.
Given a 2D radial map $\widehat{V_r}$ 
estimated by $M_r$ and supervised by GT radial maps $V_r$, 
the task is to accumulate votes, find the peak, and estimate the keypoint location.
The  
$V_r$ foreground pixels (which lie on the target object)
store the Euclidean distance from these pixels
to each of the keypoints, with background (non-object) pixels set to value $-1$. 

The estimated radial map $\widehat{V_r}$ is indeed an inverse heat map of the candidate keypoints' locations
%, as shown in Fig.~\ref{fig:v_rVSi_v_r}, 
, distributed in a radial pattern centered at the keypoints. 
% The more far away from the pixel to the keypoint,
% $\widehat{V_r}$ has a  greater value.
%The pixel is not an object pixel if $\widehat{V_r}$ is $-1$ on that pixel
To forward $\widehat{V_r}$ into a CNN voting module, 
it is inversely normalized
so that it becomes a heat map. 
Suppose that $v^{max}_r$ and $v^{min}_r$ are 
the maximum and minimum global radial distances for all objects in a dataset,
which can be calculated by iterating through all GT radial maps,
or alternately generated from the object CAD models.
An inverse radial map $\widehat{V^{-1}_r}$ can then be denoted as:
% \begin{equation}
%     \widehat{V^{-1}_r} = \frac{v^{max}_r - \widehat{V_r}}{v^{max}_r - v^{min}_r}
% \end{equation}
\begin{equation}
    \widehat{V^{-1}_r}=(v^{max}_r\!-\!\widehat{V_r})/(v^{max}_r\!-\!v^{min}_r)
\end{equation}
Thus, $M_v$ takes $\widehat{V^{-1}_r}$ as the input and 
generates the accumulated vote map 
by a series of convolution, ReLu, and batch normalization layers.
The complete network architecture is provided in the Supplementary material.
The background pixels are filtered out by a ReLu layer, 
and only foreground pixels contribute to voting.
The accumulated vote map is then max-pooled (peak extraction) 
and reshaped using a fully connected layer into a $n\! \times\! 4$ output. 
The output represents $n$ keypoints
and comprises
$n\!\times\! 2$ projected 2D keypoints $K$, 
$n$ classification labels $C$, 
and $n$ confidence scores $S$.
The labels $C$ indicate which object the corresponding keypoint belongs to, and $S$ ranks the confidence level of keypoints before being forwarded into ePnP~\cite{lepetit2009ep}
for pose estimation.
% $S_n$ is trained based on the visibility score of the objects in the scene.
%KRVNet 
$M_v$ is supervised by $\mathcal{L}_k$, $\mathcal{L}_c$, and $\mathcal{L}_s$,
and is trained end-to-end with $M_r$.







==> backup/backup-1/sec/4_exp.tex <==
\section{Experiments}
\begin{comment}
\begin{itemize}
    \item Datasets and Evaluation Metric
        LM, LMO, and YCB, as well as all BOP core datasets, 
        
        ADD(S),  0.1d, and AR of BOP 
    \item Implementation Details
        RGB and D are all normalized,
        Radii is normalized by the maximum radius,
        keypoints are projected into 2D and normalized based on the image size
        use SGD, initial lr=1e-3, reduce .1 for every n epochs
        training strategy of the network:
        1. synthetic meta-training on all classes, with four keypoints estimated
        2. take the pre-trained network on synthetic and train it on the real, with limited no. of samples and time by BOP
        3. train the adapter to pull the synthetic and real hyperspaces closer by using mmd calculated by RKHS

    
\end{itemize}
\end{comment}
\subsection{Datasets and Evaluation Metrics}
\label{sec:Datasets and Evaluation Metrics}
RKHSPose uses BOP  Procedural Blender~\cite{Denninger2023} (PBR) synthetic images~\cite{hodan2018bop,hodavn2020bop,sundermeyer2023bop,denninger2020blenderproc} for the synthetic training phase.
The images are generated 
by dropping synthetic objects (CAD models) onto a plane 
in a simulated environment using PyBullet~\cite{coumans2021}, and then rendering them
with synthetic textures.
All objects in the synthetic images are thus automatically labeled with precise GT poses. 

We evaluated RKHSPose for the six BOP~\cite{hodavn2020bop,sundermeyer2023bop} core datasets (LM (LMO)~\cite{hinterstoisser2012model}, YCB-V (YCB)~\cite{posecnn}, TLESS~\cite{hodan2017tless}, TUDL~\cite{hodan2018bop}, ITODO~\cite{drost2017introducing}, and HB~\cite{kaskman2019homebreweddb}), all except IC-BIN~\cite{doumanoglou2016recovering}, which does not include any real training and validation images and is therefore not applicable.
ITODO and HB have no real images in the training set, and so
for training 
we instead used the real images in their validation sets, which were disjoint from their test sets.
% ITODO only provides grayscale images and we forwarded the images into our model by simply reshaping the input.

% To compare with other PE methods, 
Our main results are evaluated with the ADD(S)~\cite{hinterstoisser2012model} 
metric for the LM and LMO dataset, 
and the ADD(S) AUC~\cite{posecnn} metric for the YCB dataset.
These are the standard metrics commonly used to compare 
self-supervised 6DoF PE methods.
ADD(S) is based on
the mean distance (minimum distance for symmetry) between the 
object surfaces for GT and estimated poses,
whereas ADD(S) AUC plots a curve formed by ADD(S)
for various object diameter thresholds.
We use the BOP average recall ($AR$) metrics for our ablation studies.
The $AR$ metric, based on the original ADD(S)~\cite{hinterstoisser2012model}, evaluates three aspects,
including Visible Surface Discrepancy ($AR_{VSD}$),
Maximum Symmetry-Aware Surface Distance ($AR_{MSSD}$),
and Maximum Symmetry-Aware Projection Distance ($AR_{MSPD}$).





\subsection{Implementation Details}
RKHSPose is trained on a server with an Intel Xeon 5218 CPU and 2 RTX6000 GPUs with a batch size of 32.
The Adam optimizer is used for the training of $M_{rv}$, 
on both synthetic and real data,
and $M_A$ is optimized by SGD.
Both of the optimizers have an initial learning rate of $lr\!=\!1e-3$ and weight decay $1e$-$4$ for $80$ and $20$ epochs respectively.
% $M_{rv}$ is trained for $160$ epochs on synthetic data, among which $40$ hybrid epochs (starting at epoch $120$) are combined with real data training followed by the adapter $M_A$.

The input of the network is normalized before training, as follows.
The images $I$ are normalized and standardized using ImageNet~\cite{Imagenet} specifications.
The depth maps $D$ are each individually normalized by their local minima and maxima, to lie within a range of 0 to 1.
The radial distances in radial map $V_r$ and 2D projected keypoints are both normalized by the width and height of $I$.

A single set of four keypoints is chosen by KeyGNet~\cite{wu2023learning} for the set of all objects in each dataset.
% The intermediate radial map $V_r$ is normalized by the maximum radial distance of all objects.
% The network learns 
% all categories of objects together 
% with $6$ keypoints 
% projected and normalized into 2D Image space.
One extra \emph{``background''} class is added to $C$ 
in order to filter out the redundant background points in $K$.
$M_{rv}$ is first trained for $120$ epochs on synthetic data, during which $M_A$ remains frozen. 
Following this, training proceeds for an additional $80$ epochs which alternate between real and synthetic data. When training on real data, both $M_A$ and $M_{rv}$ weights are learned, whereas $M_A$ is frozen for the alternating synthetic data training.

During real data epochs,
$M_{rv}$ initially 
estimates pseudo-keypoints for each real image. 
% initially, essentially the pseudo-keypoints.
These pseudo-keypoints are then forwarded into ePnP for pseudo-pose estimation.
Each estimated pseudo-pose 
% $p_{est}$ 
is then augmented into a set of poses $P_{aug}$,
by applying arbitrary rotational 
and translational perturbations.
Rotational perturbation
$\Delta_{R}$
and 
translational perturbation $\Delta_{T}$
% $\Delta_{R}$ and $\Delta_{T}$ is
% in the 
have respective ranges of $[-\frac{\pi}{18}, \frac{\pi}{18}]$ radians
and 
%(in the range of 
$[-0.1 , 0.1]$ 
% respectively 
along three axes 
within the normalized model frame,
which is 
defined using the largest object in the dataset.
The set of hybrid synthetic/real images
% $I_{syn/real}$
are rendered
by overlaying onto the real image the CAD model of each object 
using each augmented pose value in
$P_{aug}$.
The cardinality of
$P_{aug}$
is set to be one less than the batch size, and
the adapter $M_A$
is trained on a mini-batch of 
the hybrid images resulting from $P_{aug}$, 
plus the image resulting from the original estimated pseudo-pose.

% Specifically, $\Delta_{R}$ and $\Delta_{T}$ can be denoted as:
% \begin{equation}
%     \Delta_{R} = \{(\Delta_{\theta_i}, \Delta{\psi_i}, \Delta{\phi_i}) | \Delta_{\theta_i}, \Delta{\psi_i}, \Delta{\phi_i} \in U[-\frac{\pi}{18}, \frac{\pi}{18}]\}
% \end{equation}
% \begin{equation}
%     \Delta_{T} = {(\Delta_{x_i}, \Delta_{y_i}, \Delta_{z_i}) | \Delta_{x_i}, \Delta_{y_i}, \Delta_{z_i} \in [-0.1, 0.1]]}
% \end{equation}


Initially
$M_A$ is frozen,
and
for the first $80$ epochs,
%   during which $M_A$ is frozen,
the loss is set to emphasize the classification and the visibility score regression, i.e. $\lambda_c\!=\!\lambda_s\!=\!0.6$ and $\lambda_r\!=\!\lambda_k\!=\!0.4$.
Following this, up to epoch $200$, the scales of losses are then exchanged to fine-tune the localization of the keypoints, i.e.
$\lambda_c\!=\!\lambda_s\!=\!0.4$ and $\lambda_r\!=\!\lambda_k\!=\!0.6$.
After epoch $120$,
$M_A$ is unfrozen each alternating epoch, and 
$\lambda_D$ is set to 1 during the remaining $M_A$ training epochs.
This training strategy, shown in Fig.~\ref{fig:diagram},
%not only 
minimizes the synthetic-to-real gap
without 
%the requirement for 
any real image GT labels, and using very few (320) real images.  
\input{tabs/tab_sum}
\input{tabs/tab_sum_bop}
\input{figs/fig-results}

\subsection{Results}
\label{sec: Results}

The results are summarized in Tables~\ref{tab:mainresults} and~\ref{tab:bop_main}.
To the best of our knowledge, 
RKHSPose outperforms all existing self-supverised 6DoF PE methods.
In Table~\ref{tab:mainresults},
on LM and LMO, our ADD(S) is $+4.2\%$ and $+2\%$ better than the second best method TexPose~\cite{chen2023texpose}.  
We compared our performance to Self6D++~\cite{wang2021occlusion},
which is the only other method that evaluated using YCB,
and made $3\%$ improvements after ICP on ADD(S) AUC.
Last but not least, 
our performance evaluated on the other four BOP core datasets 
is comparable to several 
SOTA methods 
from the BOP leaderboard,
which are fully supervised with real
labels
(Table~\ref{tab:bop_main}).
Some test scenes with RKHSPose results are shown in Fig.~\ref{fig:results}.

% RKHSPose runs at 34 fps on 
% % a desktop with 
% an Intel i7 2.5GHz CPU and an RTX 3090 GPU with 24G VRAM.
% Specifically,
% it takes on average $8.7$~ms for loading data, $4.5$~ms for forward inference through $M_{rv}$, and $16.2$~ms for ePnP.
RKHSPose runs at 34 fps on 
% a desktop with 
an Intel i7 2.5GHz CPU and an RTX 3090 GPU with 24G VRAM.
It takes on average $8.7$~ms for loading data, $4.5$~ms for forward inference through $M_{rv}$ ($\times10$ faster compared to the analytical radial voting in RCVPose), and $16.2$~ms for ePnP.













==> backup/backup-1/sec/5_abla.tex <==
\section{Ablation Studies}
\label{sec: Ablation Studies}
% \subsection{Various Votings}
% \label{sec: Various Votings}
% \begin{itemize}
%     \item Voxel Voting
%     vote on a 3D voxel space, iterate through each voxel, count the votes for each voxel, and find the maxima.
%     \item RANSAC Voting
%     \item Conv Voting
%     apply conv layers on the estimated radii map; the network output is projected keypoints in 2D.
% \end{itemize}
% \input{tabs/tab_voting_schemes}

\subsection{Dense Vs. Sparse Adapter}
\label{sec: Dense VS. Sparse Discriminator}
% \begin{itemize}
%     \item apply adapter to each of the layers' output tensors comparing to an adapter on output, network depths are similar,
%     show the performance differences
% \end{itemize}
%\input{tabs/tab_disciminator_mod}
\input{tabs/tab-discriminator-mod+train-strategy}
The Adapter $M_A$ densely matches the intermediate feature maps, whereas the majority of other methods~\cite{tan2023smoc,deng2020self,wang2020self6d} only compare the final output.
In order to show the benefits of dense comparison,
we conduct an experiment with different
variations of $M_A$.
A sparse matching $M^s_A$ network is trained on synthetic and real data
comparing only 
a single feature map,
which is the intermediate radial map.
%, is trained.
$M^s_A$ has the exact same overall learning capacity (number of 
%layers and 
parameters) as the dense matching $M_A$ described in Sec.~\ref{sec: Keypoints ConvRVoting}. The results in Table~\ref{tab:discriminator desntiy}
show that
$M_A$ surpassed $M^s_A$ on all six datasets tested.
Specifically, on ITODD, $M_A$ is $12.1\%$ more accurate than $M^s_A$.
This experiment shows the effectiveness of our densely matched $M_A$.
%when adapting from synthetic training to real testing.

\subsection{Adapter Kernels and Metrics}
\label{sec: Discriminator Kernels Metrics}
% \begin{itemize}
%     \item compare RKHS based MMD to other statistical measures (Mahalanobis Distance, Cross Entropy,Wasserstein Distance) 
%     \item analyze the results along with the conclusion from other transfer learning papers.
% \end{itemize}
% \input{tabs/tab_kernels}
% \input{tabs/tab_metrics}
\input{tabs/tab-kernels+metrics}
We use linear (dot product) kernel and MMD in RKHS for domain gap measurements.
There are various other kernels and similarity measurements that can be implemented in RKHS as
described in Sec.~\ref{sec: Convolutional RKHS Discriminator}. 
First, we add trainable weights to the radial basis function (RBF) kernel in a similar manner as $K_w$ defined in Eq.~\ref{eq:kw}. 
The trainable RBF kernel on two sets of data $X$ and $Y$ is denoted as:
\begin{equation}
    K_{rbf}(X, Y) = exp(-w\left \|  X-Y\right \|^2)
\end{equation}
where $w$ are the trainable weights,
which replaces the original adjustable parameter in the classical RBF kernel.
%, we have proved the theoretical feasibility.
We also experiment with the classical RKHS kernel functions without trainable weights,
including the inner product kernel and the original RBF kernel~\cite{vert2004primer},
for comparison.
Further, we experiment on other commonly used distance measures,
including Kullback-Leibler Divergence (KL Div, i.e. relative-entropy) and Wasserstein (Wass) Distance.

In Table~\ref{tab:kernels}, the RBF kernel performs similar to the linear product kernel with a slight performance dip.
In Table~\ref{tab:metrics}, MMD minimizes the domain gap better than the Wass Distance, followed by the KL Div metric, leading to a better overall performance on $AR$.
Based on these results, we use the linear product kernel with trainable weights,
and chose 
MMD as the main loss metric in our final structure.

\input{figs/fig_no_of_reals}

\subsection{Syn/Real Synchronized Training}
\label{sec: Syn-Real Synchronized Training}
%\input{tabs/tab_train_strategy}
When training RKHSPose, real epochs are alternated with synthetic epochs. 
In contrast, some other methods~\cite{chen2023texpose,wang2020self6d,wang2021occlusion,tan2023smoc} separate the synthetic/real training.
We conducted an experiment to compare these two different training strategies,
the results of which are shown in Table~\ref{tab:train strategy}.
The alternating training performs slightly better ($+2.5\%$ on average) than the sequential training, possibly 
due to the early access to real scenes thereby avoiding local minima.
% Although the performance is relatively close, we use mixed training as there is no negative impact on the inference speed.


%\subsection{KeyGNet keypoints vs BBox and FPS}


\subsection{Number of Real Images and Real Labels}
\label{sec: No. of Real Images}

The objective of RKHSPose is to reduce real data usage and train without any real GT labels.
To show the effectiveness of the approach,
we conducted an experiment by training on different numbers of real images, 
the results of which are shown in Fig.~\ref{fig:noofreal}.
We used up to 640 real images in all cases, 
except for that of ITODD which contains
only 357 real images.
The $AR$ of all datasets saturates at 160 images except YCB. 
The further improvement of YCB beyond 160 images is also only $+0.1\%$ and saturates after 320 real images. 
We nevertheless conservatively use $320$ real unlabeled images for our main results.
This experiment also showed that adding an equal number of real labeled images beyond 320, did little to improve performance.




==> backup/backup-1/sec/6_conclusion.tex <==
\section{Conclusion}
% \begin{itemize}
%     \item summarize
%     propose a semi-supervised 6DoF PE method using rkhs and a novel architecture densely comparing the feature maps
%     shortage: can only estimate pose for a fixed amount of instances in a scene due to the design of network architecture but more accurate
    
% \end{itemize}
To sum up, we propose a novel self-supervised keypoint radial voting-based 6DoF PE method using RGB-D data called RKHSPose.
RKHSPose fine-tunes poses pre-trained on synthetic data by densely matching features with a learnable kernel in RKHS, 
using real data albeit without any real GT poses.
By applying this DA technique in feature space, 
RKHSPose achieved SOTA performance on six BOP core datasets, surpassing 
the performance of all other self-supervised methods.
Notably, the RKHSPose performance closely approaches that of several fully-supervised methods, which indicates the strength of the approach at reducing the sim2real domain gap for this problem.

% In future work, we will explore the extension of these methods to the problem of novel object 6DoF PE, in which initial CAD models of the target objects are unavailable during training.
%, so that poses can be estimated for any object in an image.
\vspace{5mm}

%keep in case required by submission
% \noindent{\bf Limitations: }A limitation of RKHSPose is that it relies on the accuracy of estimated pseudo-keypoints, 
% which at the beginning of the training process, are initially generated purely from processing synthetic data, and therefore
% depend upon the similarity between the domains of the real and synthetic images. If this domain gap is too large,
% then the initial pseudo-keypoints could be inaccurate, which could degrade performance.

\subsubsection*{Acknowledgements:}Thanks to Bluewrist Inc. and NSERC for their support
of this work.
%\parskip
%\pagebreak

==> tabs/tab-discriminator-mod+train-strategy.tex <==
\begin{comment}
\begin{table}[t]
\small
% \begin{minipage}[t]{.5\columnwidth}
\begin{minipage}[t]{.49\linewidth}
\centering

\caption{Average $AR$ of different Adapters on LM and six BOP core datasets.\label{tab:discriminator desntiy}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{3}c}
\hline
Adapter  & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
$M^s_A$ &78.1&77.8&77.8&77.9\\\hline
$M_A$ & 84.9&84.1&84.3&\textbf{84.4}\\\hline

\end{tabular}
\end{adjustbox}
\end{minipage}
\begin{minipage}[t]{.49\linewidth}
\centering

\caption{The average $AR$ of different Training Strategies on LM and five BOP core datasets.\label{tab:train strategy}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{3}c}
\hline
Training Type& $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
Mixed &84.9&84.1&84.3&\textbf{84.4}\\\hline
Sequantial&82.3&81.7&81.7&81.9\\\hline
\end{tabular}
\end{adjustbox}
\end{minipage}
% } %\raisebox
\end{table}
\end{comment}

\begin{table}[t]
\small
% \begin{minipage}[t]{.5\columnwidth}
\begin{minipage}[t]{.47\linewidth}
\centering
\caption{
%Average 
$AR$ of different adapters on LM and five BOP core datasets.\label{tab:discriminator desntiy}}
% \begin{adjustbox}{max width=0.95\columnwidth}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{ccccc}
\hline
Adapter  & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline
$M^s_A$ &78.1&77.8&77.8&77.9\\
$M_A$ & 84.9&84.1&84.3&\textbf{84.4}\\\hline
\end{tabular}
\end{adjustbox}
\end{minipage}
\hspace{0.05\linewidth}
\begin{minipage}[t]{.47\linewidth}
\centering
\caption{
%Average 
$AR$ of different training strategies on LM and five BOP core datasets.\label{tab:train strategy}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{ccccc}
\hline
Training Type& $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline
Mixed &84.9&84.1&84.3&\textbf{84.4}\\
Sequantial&82.3&81.7&81.7&81.9\\\hline
\end{tabular}
\end{adjustbox}
\end{minipage}
% } %\raisebox
\end{table}

==> tabs/tab-kernels+metrics.tex <==
\begin{comment}
\begin{table}[t]
\small
% \begin{minipage}[t]{.5\columnwidth}
\begin{minipage}[t]{.49\linewidth}
\centering
\caption{Average $AR$ of different RKHS kernels on LM and five BOP core datasets.\label{tab:kernels}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c|cV{3}c}
\hline
Kernels&$w$ & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
\multirow{+2}{*}{Linear}& \redxmark& 71.6&	70.8&	70.6&	71.0\\\cline{2-6}
& \greencheckmark&84.9&84.1&84.3&\textbf{84.4}\\\cline{1-6}
\multirow{+2}{*}{RBF} & \redxmark &  73.4&	72.9&	73.2&	73.2 \\\cline{2-6}
  &\greencheckmark&82.5&81.3&81.5&81.6\\\hline
\end{tabular}
\end{adjustbox}
\end{minipage}
\begin{minipage}[t]{.49\linewidth}
\centering
\caption{Average $AR$ of different metrics on LM and five BOP core datasets.\label{tab:metrics}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{3}c}
\hline
Metrics & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
MMD &84.9&84.1&84.3&\textbf{84.4}\\\hline
KL Div&78.0&77.8&78.0&77.9\\\hline
Wass Distance&80.9&80.6&80.9&80.8\\ \hline
\end{tabular}
\end{adjustbox}
\end{minipage}
% } %\raisebox
\end{table}
\end{comment}
\begin{table}[t]
\small
% \begin{minipage}[t]{.5\columnwidth}
\begin{minipage}[t]{.48\linewidth}
\centering
\caption{
%Average 
$AR$ of different kernels on LM and five BOP core datasets.\label{tab:kernels}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{cccccc}
\hline
Kernel&$w$ & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline
\multirow{+2}{*}{Linear}& \redxmark& 71.6&	70.8&	70.6&	71.0\\%\cline{2-6}
& \greencheckmark&84.9&84.1&84.3&\textbf{84.4}\\%\cline{1-6}
\multirow{+2}{*}{RBF} & \redxmark &  73.4&	72.9&	73.2&	73.2 \\%\cline{2-6}
  &\greencheckmark&82.5&81.3&81.5&81.6\\\hline
\end{tabular}
\end{adjustbox}
\end{minipage}
\hspace{0.05\linewidth}
\begin{minipage}[t]{.47\linewidth}
\centering
\caption{
%Average 
$AR$ of different metrics on LM and five BOP core datasets.\label{tab:metrics}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{ccccc}
\hline
Metric & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline%\hline
MMD &84.9&84.1&84.3&\textbf{84.4}\\%\hline
KL Div&78.0&77.8&78.0&77.9\\%\hline
Wass Distance&80.9&80.6&80.9&80.8\\ \hline
\end{tabular}
\end{adjustbox}
\end{minipage}
% } %\raisebox
\end{table}


==> tabs/tab_bop_ours.tex <==
\begin{table}[t]
\begin{center}
\caption{RKHSPose results evaluated by BOP $AR$ metric~\cite{hodan2018bop,hodavn2020bop,sundermeyer2023bop} on LM and six BOP core datasets with real images. Our performance on some datasets compare with the SOTA methods on BOP leaderboard with full supervision of real labels.\label{tab:bop_main}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{2.5}c}
\hline
 Dataset  & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
 LM & 96.0&95.7&95.7&95.8 \\ \hline
LMO  &  68.7  &   68.2  &  68.2&68.4   \\  \hline
 T-LESS    &    85.9     & 85.1&85.8 &  85.6  \\ \hline
 TUD-L  &  \textbf{97.6}       & \textbf{96.4}&\textbf{95.4}  & \textbf{96.2} \\ \hline
 %IC-BIN &   73.5  & 71.4 &72.8  &   72.6  \\  \hline
 ITODD    &   69.2    &68.5  & 68.4   & 68.7 \\ \hline
 HB &   \underline{92.7}&\underline{91.6}      &  \underline{92.5}  & \underline{92.3}\\ \hline
 YCBV &     83.9&83.4    &  84  & 83.8\\ \hline
\end{tabular}
\end{adjustbox}


\end{center}
\end{table}

==> tabs/tab_disciminator_mod.tex <==
\begin{table}[t]
\begin{center}
\caption{Average $AR$ of different Adapters on LM and five BOP core datasets.\label{tab:discriminator desntiy}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{3}c}
\hline
Adapter  & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
$M^s_A$ &78.1&77.8&77.8&77.9\\\hline
$M_A$ & 84.9&84.1&84.3&\textbf{84.4}\\\hline

\end{tabular}
\end{adjustbox}


\end{center}
\end{table}

==> tabs/tab_epnpvshorn.tex <==
\begin{table}[t]
\begin{center}
\caption{EPnP vs. Horn's method: EPnP taking 2D-3D correspondences as input performs slightly better/exactly the same compared to 3D correspondences based Horn's method on all datasets except HB.
\label{tab:epnpvshorn}
}
%\resizebox{\columnwidth}{!}{%
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c|c|c|c|c}
\cline{2-8}
\multicolumn{1}{c|}{\multirow{2}{*}{}} 

 &
\multicolumn{7}{c}{Dataset} \\\cline{2-8}

&LM&LMO&TLESS&TUDL&ITODD&HB&YCB\\\cline{1-8}
epnp&\textbf{95.8}&\textbf{68.4}&\textbf{85.6}&\textbf{96.2}&\textbf{68.7}&92.3&\textbf{83.8}

\\\hline
horn&95.6&\textbf{68.4}&85.5&\textbf{96.2}&68.5&\textbf{92.4}&83.7

\\\hline


\end{tabular}
\end{adjustbox}

%} % \resizebox
\end{center}
\vspace{-2\baselineskip}
\end{table}


==> tabs/tab_kernels.tex <==
\begin{table}[t]
\begin{center}
\caption{Average $AR$ of different RKHS kernels on LM and five BOP core datasets.\label{tab:kernels}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c|cV{3}c}
\hline
Kernels&$w$ & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
\multirow{+2}{*}{Linear}& \xmark& 71.6&	70.8&	70.6&	71.0\\\cline{2-6}
& \checkmark&84.9&84.1&84.3&\textbf{84.4}\\\cline{1-6}
\multirow{+2}{*}{RBF} & \xmark &  73.4&	72.9&	73.2&	73.2 \\\cline{2-6}
  &\checkmark&82.5&81.3&81.5&81.6\\\hline
\end{tabular}
\end{adjustbox}


\end{center}
\end{table}

==> tabs/tab_metrics.tex <==
\begin{table}[t]
\begin{center}
\caption{Average $AR$ of different metrics on LM and five BOP core datasets.\label{tab:metrics}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{3}c}
\hline
Metrics & $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
MMD &84.9&84.1&84.3&\textbf{84.4}\\\hline
KL Div&78.0&77.8&78.0&77.9\\\hline
Wass Distance&80.9&80.6&80.9&80.8\\ \hline
\end{tabular}
\end{adjustbox}


\end{center}
\end{table}

==> tabs/tab_train_strategy.tex <==
\begin{table}[t]
\begin{center}
\caption{The average $AR$ of different Training Strategies on LM and five BOP core datasets.\label{tab:train strategy}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|cV{3}c}
\hline
Training Type& $AR_{VSD}$ & $AR_{MSSD}$ & $AR_{MSPD}$ & $AR$\\ \hline\hline
Mixed &84.9&84.1&84.3&\textbf{84.4}\\\hline
Sequantial&82.3&81.7&81.7&81.9\\\hline
\end{tabular}
\end{adjustbox}


\end{center}
\end{table}

==> tabs/tab_voting_schemes.tex <==
\begin{table}[t]
\begin{center}
\caption{The impact of different votings\label{tab:votingSchemes}}
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{c|c|c|c|c}
\cline{3-5}
\multicolumn{2}{c}{} &\multicolumn{2}{|c|}{$\bar{\epsilon}$ [mm]}& speed \\\hline
Refine & Voting Type  & $\mu$ & $\sigma$ &fps\\ \hline\hline
\multirow{+3}{*}{No} & Voxel   Voting  &    &     &     \\  \cline{2-5}
 & Conv   Voting    &         &  &    \\ \cline{2-5}
 & RANSAC   Voting  &         &   &  \\ \hline
\multirow{+3}{*}{Yes} & Voxel   Voting  &     &    &     \\  \cline{2-5}
 & Conv   Voting    &         &    &  \\ \cline{2-5}
 & RANSAC   Voting  &         &    & \\ \hline
\end{tabular}
\end{adjustbox}


\end{center}
\end{table}
